Deep Value Networks Learn to Evaluate and Iteratively Refine Structured Outputs

We approach structured output prediction by optimizing a deep value network (DVN) to precisely estimate the task loss on different output configurations for a given input. Once the model is trained, we perform inference by gradient descent on the continuous relaxations of the output variables to find outputs with promising scores from the value network. When applied to image segmentation, the value network takes an image and a segmentation mask as inputs and predicts a scalar estimating the intersection over union between the input and ground truth masks. For multi-label classification, the DVN's objective is to correctly predict the F1 score for any potential label configuration. The DVN framework achieves the state-of-the-art results on multi-label prediction and image segmentation benchmarks.

==> details.tex <==
\label{details}
\begin{figure}[t]
\includegraphics[width=\linewidth]{net_small.pdf}
\caption{A deep value network that takes 
an image and a segmentation mask as input and predicts a scalar
evaluating the compatibility between the input pairs.}
\label{fig:arch}
\end{figure}
\subsection{Implementation details}
For our value network we use a simple CNN architecture consisting of 3 convolutional and 2 fully connected layers (Figure~\ref{fig:arch}).
We use a learning rate of $0.01$ and apply dropout on the first fully connected layer with the keeping probability $0.75$ as determined on the validation set. For stratified sampling we empirically found $\tau=0.05$ to work best.

For training data augmentation purposes we randomly crop the image, similar 
to~\cite{krizhevsky2012imagenet}.
At test time, various strategies are possible to obtain a fully resolution 
segmentation, which we investigate in Section~\ref{sec:ablation}.
If not explicitly stated, masks are averaged over over 36 crops for our model and~\cite{long2015fully} (see below).

For comparison we also implemented a fully convolutional network baseline~\cite{long2015fully}, by using a similar architecture as for the value network.
To obtain per-pixel prediction we transformed the fully connected layers to convolutions and extended the network with learnt upscaling layers (transposed convolutions) initialized to bilinear interpolation.
We combined the predictions from the last layer with the predictions based on the second convolutional layer to be able to predict finer details, while retaining high-level semantic information~\cite{long2015fully}.

